Foraging for dark matter in large volume liquid scintillator neutrino detectors with multiscatter events

We show that dark matter with a per-nucleon scattering cross section $\gtrsim 10^{-28}~{\rm cm^2}$ could be discovered by liquid scintillator neutrino detectors like BOREXINO, SNO+, and JUNO. Due to the large dark matter fluxes admitted, these detectors could find dark matter with masses up to $10^{21}$ GeV, surpassing the mass sensitivity of current direct detection experiments (such as XENON1T and PICO) by over two orders of magnitude. We derive the spin-independent and spin-dependent cross section sensitivity of these detectors using existing selection triggers, and propose an improved trigger program that enhances this sensitivity by two orders of magnitude. We interpret these sensitivities in terms of three dark matter scenarios: (1) effective contact operators for scattering, (2) QCD-charged dark matter, and (3) a recently proposed model of Planck-mass baryon-charged dark matter. We calculate the flux attenuation of dark matter at these detectors due to the earth overburden, taking into account the earth's density profile and elemental composition, and nuclear spins.

==> universalnewcommands.tex <==
\newcommand{\half}{\frac{1}{2}}
\newcommand{\gsim}{\gtrsim}
\newcommand{\lsim}{\lesssim}
\newcommand{\ra}{\rightarrow}
\newcommand{\mtop}{m_t}
\newcommand{\ct}{c_\theta}
\newcommand{\st}{s_\theta}
\def\sigmaveeave{\langle \sigma v\rangle}
\def\sigmaveeann{\langle \sigma v\rangle_{\rm ann}}
\def\relabund{\Omega_\chi h^2}
\def\lag{\mathcal{L}}
\def\Oc{\mathcal{O}}
\def\Mc{\mathcal{M}}
\def\shat{\sqrt{\hat{s}}}
\def\shatsq{\sqrt{s}}
\def\met{\slashed{E}_T}


\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\nn}{\nonumber}
